Polynomial Kernels for Generalized Domination Problems

In this paper, we study the parameterized complexity of a generalized domination problem called the [${\sigma}, {\rho}$] Dominating Set problem. This problem generalizes a large number of problems including the Minimum Dominating Set problem and its many variants. The parameterized complexity of the [${\sigma}, {\rho}$] Dominating Set problem parameterized by treewidth is well studied. Here the properties of the sets ${\sigma}$ and ${\rho}$ that make the problem tractable are identified [1]. We consider a larger parameter and investigate the existence of polynomial sized kernels. When ${\sigma}$ and ${\rho}$ are finite, we identify the exact condition when the [${\sigma}, {\rho}$] Dominating Set problem parameterized by vertex cover admits polynomial kernels. Our lower and upper bound results can also be extended to more general conditions and provably smaller parameters as well.

==> EDS_Parameterized_by_Modular_Width.tex <==
\section{FPT algorithm by Modular width}
\begin{theorem}\label{EDSMod}
For every graph connected $G=(V,E)$ with modular width $mw$, \eds is solvable in $O(2^mw . n^c)$ time. 

\end{theorem}

\begin{proof}
We compute the modular decomposition tree $\mathcal{M}$ of $G$. We traverse tree in bottom up manner and for every node $M_t$ in $\mathcal{M}$, we consider the subgraph $G_t$ of $G$ that corresponds to $M_t$ and returns the efficient dominating set of $G_t$, it it exists or else returns $NULL$. We know that every node in $\mathcal{M}$ is one of four types. We explain the algorithm for each type of the tree as follows.

%for each $v_M$ in $MD(G)$, with M denoting the corresponding module of $G$, we will compute dominating set. For root module $v_M$ of $MD(G)$, $G[M]=G$. Any module $v_M$ is either of the four operation.
\begin{enumerate}
\item{Introduce node : }
This node introduces a vertex $v$ as an isolated vertex. $v$ can be efficiently dominated by selecting $v$ into the dominating set.
\item{Disjoint Union operation :}
A disjoint union node $t$ corresponds to the disjoint union of two graphs $G_1$ and $G_2$ that corresponds to the child nodes of $t$. The efficient dominating set exists for the larger graph if and only if efficient dominating set exists for both $G_1$ and $G_2$ and is given by the union of their solutions. 


\item{Complete Join Operation :}
A join node $t$ corresponds to the join of two graphs $G_1$ and $G_2$ that corresponds to the child nodes of $t$. Now for all $u \in V(G_1)$ and $v \in V(G_2)$, $u$ and $v$ are adjacent in $G$. Therefore, if $D$ is an efficient dominating set of $G$, then $D$ cannot contain two vertices from $G_1$ or two vertices from $G_2$ or one each from $G_1$ and $G_2$. Thus the only case where $D$ exists is when either $G_1$ or $G_2$ contains a vertex which is adjacent to every other vertex in $G$. We can find if such a vertex exists in linear time.
\item{Substitution Operation :}
A substitution node substitutes the child nodes $G_1$, $G_2$, \dots, $G_m$ in a base graph $B$ with $m$ vertices to get the graph $G$. Since $G$ is a connected graph, a dominating set $D$ of $G$ cannot contain two vertices from any $G_i$. Also, if $G_i$ and $G_j$ are adjacent in $G$, $D$ cannot contain one vertex each from $G_i$ and $G_j$. Therefore, if a vertex $v \in V_i$ belongs to $D$, then $v$ should also dominate every vertex in $V_i$ and therefore $v$ should be a universal vertex of $G_i$. The algorithm checks every $G_i$ to see if there exists a universal vertex in $G_i$. Then the algorithm iterates through every subset of at most $m$ universal vertices and check if it is an efficient dominating set of $G$. This step takes $O(2^m)$ time.
\end{enumerate}
Now the result follows. 


\end{proof}

\begin{theorem}

 The \ptds problem parameterized by modular width admits FPT algorithm with running time $O(2^mw . n^c)$

\end{theorem}

\begin{proof}
The proof is similar to that of Theorem~\ref{EDSMod}. We explain the algorithm for each of the four types of nodes of the modular decomposition tree. 
\begin{enumerate}
\item{Introduce node :}  An isolated vertex cannot be dominated by a total perfect dominating set. Therefore, the algorithm returns $NULL$.
\item{Disjoint Union Node : } This is handled in the same way as before.
\item{Complete Join Node:} If $D$ is a perfect total dominating set of $G$, then $D$ cannot contain two vertices from $G_1$ (or $G_2$) since that means vertices in $G_2$ have two neighbours in $D$. Assume the vertex $u$ from $G_1$ belongs to $D$. Every vertex in $G_2$ is dominated by $u$. Now $u$ needs to be dominated by another vertex, let that be $v$ from $G_2$. Since evrey vertex in $G_2$ is already dominated by $u$, they cannot be adjacent to $v$. Hence, $v$ (resp. $u$) is an isolated vertex in $G_1$ (resp. $G_2$). Therefore, the algorithm checks if there exists an isolated vertex in $G_1$ and $G_2$.
\item{Substitution operation : If a perfect total dominating set exists, then every $G_i$ contains at most one vertex from $D$ and if it exists, then that is an isolated vertex in $G_i$. Thus the algorithm checks every $G_i$ for an isolated vertex and then iterates over all subsets of at most $m$ isolated vertices in $O(2^m)$ time. } 
\end{enumerate}
\end{proof}

%\begin{theorem}

% The \pds problem parameterized by modular width admits FPT algorithm with running time $O(2^mw . n^c)$
%
%\end{theorem}
%
%\begin{proof}
%
%\end{proof}


==> conclusion.tex <==
\section{Conclusion}
 
We studied the \sirho problem for existence of polynomial kernels for structural parameters such as Vertex Cover, Degree d modulator and Neighborhood Diversity. Among other results we proved the \sirho problem for bounded $\sigma , \rho $ when parameterized by vertex cover admits a polynomial kernel if and only if $\sigma \cap \rho = \emptyset$. It would be interesting to study if the results can be extended to   cases when $[\sigma, \rho]$ is unbounded and also for maximization variants.

==> girth_5_perfect_domi.tex <==
\section{In Girth $\geq $ 5 Graphs.}

\begin{lemma} \label{g5ik}
\pds has a kernel of $O(k^3 * log k )$ in girth $\geq $ 5 Graphs (Graphs which don't have cycles of length 3 and 4).
\end{lemma}

\begin{proof}

We follow the proof from \cite{perf} and add a reduction to Weighted Perfect Dominating Set.In the \cite{perf} \pds is semi-perfect code .\\


In \cite{perf} they convert this problem to RWB-Dominating Set problem and prove Theorem \ref{g5pr} 

\defproblem{{RWB-Dominating Set} }{Given a graph G whose vertex set V is partitioned
into $R_G, W_G,$ and $B_G$ (colored red, white, and black, respectively) and parameter k }{is there a subset $S \subseteq V$ of size at most k such that
$R_G \subseteq S$ and S dominates $B_G$. 
}

We use Theorem \ref{g5pr} which is proved in \cite{perf}.

\begin{theorem} \label{g5pr}
The Problem can be reduced such that the Number of Red vertices is at most $k$,black vertices is at most $k^2$, number of white component is $k^3$ and each white component has at most white k vertices.Hence number of white vertices is at most $k^4$
\end{theorem}

Here white component means maximal connected component consisting of only white vertices.

We reduces to Weighted Perfect Dominating $G'$ by merging every white component lets say $W_i$ into single vertex $w_i$ with weight equal to  $|W_i|$ vertex. This is because if one white vertex of a white component is selected then all white vertex from that component must be selected. Now if there was a black vertex $u$ such that$ | N(u) \cap W_i | > 1 $ then we add a special edge of color green between the $ w_i$ and $u$ which signifies that if we select $w_i$ we must select u into D as $ | N(u) \cap W_i | > 1 $. 

\begin{lemma}If G has a \pds of size $k$ them G' has a weighted \pds* of weight k and vice versa \label{perfec}

\end{lemma}

\begin{proof}
If $G$ has a \pds of size k then the weighted perfect dominating set of $G'$ contains $\{u : (u \in D) \wedge (u \notin W_G)\} \cup \{w_i : (v \in D) \wedge (v \in W_i)\}$.
If $G'$ has a weighted perfect dominating set of weight k then \pds of $G$ is $\{v :( v \in D') \wedge (v \in V(G)) \}  \cup  \{v : v \in W_i  \wedge  w_i  \in D' \}$

\end{proof}

We know there are atmost $k^3$ white component hence number of white vertices in $G'$ is $(k^3)$. We observe that weight of each white vertex is at most k hence it requires at most $log k$ space to store.Hence it admits a kernel of size $O(k^3 * log k )$ bits .

\end{proof}


==> girth_5_perfect_total.tex <==
\begin{lemma}
Weakly-perfect code and \ptds has a kernel of size $O(k^3)$
\end{lemma}{.}

We convert into  RWB-Dominating Set and continue from Theorem \ref{g5pr}.

we add a reduction rules to the proof given by \cite{perf}.

\begin{itemize}
    \item if white vertex has white neighbours we can delete all these white vertices as these white vertices can never be selected in dominating set.
    
    \item If two red vertices u and v are adjacent to the same red vertex w, return no.
\end{itemize}

We see that number of white vertices is $O(k^3)$.

Similar argument to proof of Lemma \ref{g5ik}.

==> poly_kernel.tex <==
\section{Polynomial Kernel Results}

We show that \eds when parameterized by vertex cover has a kernel of $O(k^4)$ were k is the size of vertex cover.We show this by solving a more general problem that is \geds  .Given a graph G domination[i,i] asks if there exists a set D such that $\forall v \in V,  |N[v] \cap D| = i$ .So when $i = 1$ domination[i,i] is equivalent to \eds

\begin{lemma}
For any fixed i , \geds when parameterized by vertex cover has a kernel of $O(k^4)$ bits where k is the size of Vertex Cover
\end{lemma}

We follow the method given from \cite{3-cncf} section 4.3 for kernalization of 2-CNCF-Coloring.\\

We convert our problem instance of \geds to an equivalent instance \dpoly .We will then carefully rephrase the \dpoly instance such that it uses only a limited number of variables, such that we can use a known kernelization result \ref{d-poly} for \dpoly to obtain our desired compression.\\
\dpoly over a field F is defined as.
\begin{tcolorbox}
Input: A list L of polynomial qualities over variables $V = \{x_1,...,x_n\}$. An
equality is of the form $f(x_1,\cdots,x_n) = 0$, where f is a multivariate polynomial
over F of degree at most d.\\
Question: Does there exist an assignment of the variables $\tau: V \rightarrow \{0, 1\}$
satisfying all equalities (over F) in L?
\end{tcolorbox}

\begin{theorem} \label{d-poly}
There is a polynomial-time algorithm that,
given an instance (L, V ) of d-Polynomial ROOT CSP over an efficient field F ,outputs an equivalent instance (L',V) with at most $n^d + 1$ constraints such that L' $\subseteq$ L.
\end{theorem}

\begin{proof}

Given an instance G with vertex cover S of size k we create an instance of \dpoly where d is 2 that is satisfiable if and only if G has a \geds.Let V := $\{s_{v}  | v \in V(G) \}$ ( s - selected in \geds) be variable set. We create L over $\mathbb{Q}$  as follow

\begin{enumerate}
    \item For each $v \in V(G)$, add the  $(s_{v} - 1)(s_v) = 0$ to L.
    
    \item For each $v \in V(G)$, add the  $(-i + \sum_{u \in N[v]} s_u) = 0$
  
\end{enumerate}
We add the first equation to ensure that either the vertex is selected in \geds or not.The second equation ensures that exactly $i$ vertices in the closed neighbourhood of v is selected.

\begin{lemma}
$(L,V)$ is a yes-instance of 2-Polynomial ROOT CSP if and only G has a \geds set D.
\end{lemma} 

\begin{proof}
Suppose  $\tau$ : V $\rightarrow$ $\{0, 1\}$ is a satisfying assignment for $(L, V )$. We show how to select vertices for \geds of G.Vertex v is selected if and only if $\tau (s_{v})$ = 1 and vertex v is not selected if and only if $\tau (s_{v})$ = 0. because of,Step 1, $(s_{v} - 1)(s_v) = 0$ this ensure exactly one state for each vertex v.Now we show that it is indeed \geds.Let $v \in V(G)$ be an arbitrary vertex we show that $N[v]$ follows \geds rules.From, equation added in step 2.
$ \sum_{u \in N[v]} s_u) = i $ this shows that $N[v]$ contains exactly $i$ vertex which is selected.\\


This concluded this direction of proof.\\

For other direction, Suppose G has \geds set we show how to define a satisfying assignment $\tau$ for (L,V). For v $\in$ V (G), let $\tau (s_{v}) := 1$  if v is in the dominating set and let  $\tau (s_{v}) := 0$ otherwise.Observe that by this definition, $\tau(s_{v})= 1$ or $\tau(s_{v}) = 0$  for a $v \in V(G)$ ,showing that we satisfy all equation introduced in step 1. For the
equations introduced in Step 2, consider an arbitrary vertex $v \in V (G)$, then exactly $i$ element from $N[v]$ is selected hence $ \sum_{u \in N[v]} s_u) = i $ .\\

\end{proof}

We see that $|V| = n$ if n is the number of vertices of G. We will modify L,such that it uses only variables for the vertices in S.To do this, we introduce a function.For $v \notin
S$,let $f_{v} = g(\sum_{u \in N(v)} s_u)$ where

$$g(x) = i - x$$

is a degree 1 function.\\

Observe that $f_v$ only uses variable defined for vertices that are in S.Let $L'$ be equal to $L$ with every occurrence of $s_v$ for $v \notin S$ substituted by $f_v$.\\

\begin{lemma}
If $\tau: V \rightarrow \{0, 1\}$ is a satisfying assignment for $(L, V )$, then $\tau|v'$
is a satisfying assignment for $(L', V')$
\end{lemma}.

\begin{proof}
We show this by showing that for all $v \notin S$ , $f_v(\tau(V )) = \tau(s_v)$ in this case.Since $s_v = 1 $ or $s_v = 0$ by equations added in Step 1, Consider an arbitrary vertex v $\notin$ S Observe that by the equation added in step 2 ,one of the cases happens 

\begin{enumerate}
    \item $s_v = 1$ , as $\sum_{u \in N[u] } s_{u} = i$.In this case $\sum_{u \in N(u)} s_{u} = i - 1$ and thereby $f_v = g(i-1) = 1 = s_v$.
    \item $s_v = 0$ , as $\sum_{u \in N[u] } s_u = i$.In this case $\sum_{u \in N[u] } s_u= i$ and thereby $f_v = g(i) = 0 = s_v$.
\end{enumerate}

\end{proof}

Equivalence between $(L',V')$ and $(L,V)$ can be proven in similar way .\\

We have obtained $(L',V')$ which is satisfiable if and only if $(L, V )$ is satisfiable.Observe that $|V'| = O(k)$ as it contains only variables of vertex cover vertices


In $L'$ has at most k variables and have degree at most 2 . We use Theorem 7 to obtain $L_1'' \subseteq L'$ such that
$|L'' | = O((k^2))$ .To represent a single constraint, it is sufficient to  store the coefficient for each variable in V'.The storage space needed for a single coefficient  is $log n$ . Thereby, $(L'', V '')$ can be stored in $O(k^{2} . k^{1} . log n)$   ,if $k \leq logn$ then we can solve trivially by guessing selected vertices from S which belong to the solution in $O(2^k * poly(n))$ Therefore we can assume  $k \geq logn$.Thereby we conclude we can $(L',V')$ can be stored in $O(k^{4})$ bits.
 
\end{proof}

==> table.tex <==
\section{Table}

\begin{center}
\begin{tabular}{ c c c }
 Parameters & Vertex cover & Neighbourhood diversity \\ 
 $\sigma = bounded$ and $\rho = unbounded$ & cell5 & ... \\  
  $\sigma = unbounded$ and $\rho = bounded$ & cell8 & polykernel $k^2$  \\
  $\sigma = bounded$ and $\rho = bounded$ &  & Linear kernel    
\end{tabular}
\end{center}

==> w_hard_bipartite.tex <==
\begin{lemma}
\ptds is W[1] in bipartite graph.
\end{lemma}

We follow similar proof of  perfect code is W[1] hard from \cite{perf}.

The proof uses FPT reductions based on the same construction from the $W[1]$-hard problem multicolored \clq.

\begin{proof}
Given a graph $G = (V,E)$ and a vertex-coloring $\kappa : V \rightarrow \{1, 2,\cdots,k\}$, multicolored \clq is the problem of deciding whether G has a \clq of k vertices
containing exactly one vertex of each color. Let $V_{i}$ be the set of vertices in G with
color i, $1 \leq i \leq k$. Assume without loss of generality that there are no edges between
vertices in $V_i$. Fix an ordering of the vertices in each $V_i$. For $u, v \in V_{i}$, let $u<v$
denote that the index of u is less than the index of v in the fixed ordering. Let $E_{i,j}$
be the set of edges in G between $V_{i}$ and $V_j$ , $1 \leq i < j \leq k$.

Given an input graph G = (V,E) for multicolored clique, we construct an input
graph $G' = (V', E')$ for the \ptds as follows. $G'$ contains a vertex selection
gadget for each $V_i$, an edge selection gadget for each $E_{i,j}$ , and a validation gadget
for each ordered pair $(V_{i}, V_{j} )$, $1 \leq i < j \leq k$.

For each vertex set $V_{i}$, we construct a vertex selection gadget which is itself a bipartite graph,we add 3 vertices $x_{i}^1 , x_{i}^{2} , x_{i}^3$ .$V_i$ is spilt into two parts $\{v| v \in V_{i}\} \cup \{x_{i}^{1}\}$ and $\{x_{i}^{2} , x_{i}^{3}\}$. $x_{i}^{2}$ is adjacent to all vertices of first part and $x_{i}^{3}$ is adjacent to all vertices of first part except $x_{i}^{1}$.

The edge selection gadgets are constructed in a similar fashion. For each edge set $E_{i,j}$ , the edge selection gadget for $E_{i,j}$ is a bipartite graph,we add 3 vertices $t_{i,j}^{1} , t_{i,h}^{2} , t_{i,j}^{3}$  in similar manner to vertex selection gadget. 

the validation gadget is similar to the paper.

We claim that G has a k-multicolored clique if and only if $G'$ has a \ptds of size $k'= 2k + 2 \binom{k}{2} $

suppose that D is a \ptds of size k' for $G'$
. Observe , D must include exactly two vertices from each vertex selection gadget and each edge selection gadget.
We next show that the two vertices in D . Consider the vertex selection gadget for 
To dominate $x_{i}^2$ and $x_{i}^3$, D must include exactly one vertex v from the first part and $x_{i}^2 \in D$ to dominate $x_{i}^1$. Similarly,
the two vertices in D from the edge selection gadget for $E_{i,j}$ .
Consider any two vertices $u \in V_i$ and $v \in V_j$ corresponding to two pairs of
vertices u,  and v in D from the two vertex selection gadgets for $V_i$ and $V_j$ .
Observe that u dominates vertices $f_{i,j} [w]$ for $w \leq u \in V_i$, and that v dominates
vertices $f_{i,j} [w]$ for $w \leq v \in V_j$ . To perfectly dominate the remaining validation
vertices $f_{i,j} [w]$ for $w>u$ in $V_i$ and $w>v$ in $V_j$ , D must include vertex
e from the edge selection gadget for $E_{i,j}$ corresponding to the edge $e = \{u,v\}$.
Therefore, the vertices $\{v \in Vi | v, x_{i}^2 \in D, 1 \leq i \leq k\}$ form a k-multicolored \clq
K in G. 


The other direction can be proven in similar manner.

\begin{center}
\begin{frame}


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,324); %set diagram left start at 0, and has height of 324

%Shape: Circle [id:dp5989778570781332] 
\draw   (220.78,53.82) .. controls (220.78,51.11) and (222.98,48.91) .. (225.69,48.91) .. controls (228.41,48.91) and (230.61,51.11) .. (230.61,53.82) .. controls (230.61,56.54) and (228.41,58.74) .. (225.69,58.74) .. controls (222.98,58.74) and (220.78,56.54) .. (220.78,53.82) -- cycle ;
%Shape: Circle [id:dp1969403674772814] 
\draw   (220.11,93.82) .. controls (220.11,91.11) and (222.31,88.91) .. (225.03,88.91) .. controls (227.74,88.91) and (229.94,91.11) .. (229.94,93.82) .. controls (229.94,96.54) and (227.74,98.74) .. (225.03,98.74) .. controls (222.31,98.74) and (220.11,96.54) .. (220.11,93.82) -- cycle ;
%Shape: Circle [id:dp4862352837629178] 
\draw   (260.44,24.16) .. controls (260.44,21.44) and (262.65,19.24) .. (265.36,19.24) .. controls (268.08,19.24) and (270.28,21.44) .. (270.28,24.16) .. controls (270.28,26.87) and (268.08,29.07) .. (265.36,29.07) .. controls (262.65,29.07) and (260.44,26.87) .. (260.44,24.16) -- cycle ;
%Shape: Circle [id:dp48408840152077426] 
\draw   (260.44,53.82) .. controls (260.44,51.11) and (262.65,48.91) .. (265.36,48.91) .. controls (268.08,48.91) and (270.28,51.11) .. (270.28,53.82) .. controls (270.28,56.54) and (268.08,58.74) .. (265.36,58.74) .. controls (262.65,58.74) and (260.44,56.54) .. (260.44,53.82) -- cycle ;
%Shape: Circle [id:dp6878965314508212] 
\draw   (260.44,84.16) .. controls (260.44,81.44) and (262.65,79.24) .. (265.36,79.24) .. controls (268.08,79.24) and (270.28,81.44) .. (270.28,84.16) .. controls (270.28,86.87) and (268.08,89.07) .. (265.36,89.07) .. controls (262.65,89.07) and (260.44,86.87) .. (260.44,84.16) -- cycle ;
%Shape: Circle [id:dp5991408274625996] 
\draw   (260.44,113.82) .. controls (260.44,111.11) and (262.65,108.91) .. (265.36,108.91) .. controls (268.08,108.91) and (270.28,111.11) .. (270.28,113.82) .. controls (270.28,116.54) and (268.08,118.74) .. (265.36,118.74) .. controls (262.65,118.74) and (260.44,116.54) .. (260.44,113.82) -- cycle ;
%Straight Lines [id:da5645270767900075] 
\draw    (229.94,93.82) -- (260.44,113.82) ;
%Straight Lines [id:da8217658988078178] 
\draw    (229.94,93.82) -- (260.44,84.16) ;
%Straight Lines [id:da5368453265798088] 
\draw    (229.94,93.82) -- (260.44,53.82) ;
%Straight Lines [id:da07739179115242045] 
\draw    (229.94,93.82) -- (247.26,54.27) -- (260.44,24.16) ;
%Straight Lines [id:da04050203311195966] 
\draw    (230.61,53.82) -- (260.44,84.16) ;
%Straight Lines [id:da8689345740238357] 
\draw    (230.61,53.82) -- (260.44,53.82) ;
%Straight Lines [id:da9442752019020775] 
\draw    (230.61,53.82) -- (260.44,24.16) ;
%Shape: Circle [id:dp7440194344390263] 
\draw   (222.78,199.81) .. controls (222.78,197.09) and (224.98,194.89) .. (227.69,194.89) .. controls (230.41,194.89) and (232.61,197.09) .. (232.61,199.81) .. controls (232.61,202.52) and (230.41,204.72) .. (227.69,204.72) .. controls (224.98,204.72) and (222.78,202.52) .. (222.78,199.81) -- cycle ;
%Shape: Circle [id:dp7067742172787597] 
\draw   (222.11,239.81) .. controls (222.11,237.09) and (224.31,234.89) .. (227.03,234.89) .. controls (229.74,234.89) and (231.94,237.09) .. (231.94,239.81) .. controls (231.94,242.52) and (229.74,244.72) .. (227.03,244.72) .. controls (224.31,244.72) and (222.11,242.52) .. (222.11,239.81) -- cycle ;
%Shape: Circle [id:dp7499308249193724] 
\draw   (262.44,199.81) .. controls (262.44,197.09) and (264.65,194.89) .. (267.36,194.89) .. controls (270.08,194.89) and (272.28,197.09) .. (272.28,199.81) .. controls (272.28,202.52) and (270.08,204.72) .. (267.36,204.72) .. controls (264.65,204.72) and (262.44,202.52) .. (262.44,199.81) -- cycle ;
%Shape: Circle [id:dp9147897853503391] 
\draw   (262.44,230.14) .. controls (262.44,227.42) and (264.65,225.22) .. (267.36,225.22) .. controls (270.08,225.22) and (272.28,227.42) .. (272.28,230.14) .. controls (272.28,232.85) and (270.08,235.06) .. (267.36,235.06) .. controls (264.65,235.06) and (262.44,232.85) .. (262.44,230.14) -- cycle ;
%Shape: Circle [id:dp6491671744645766] 
\draw   (262.44,259.81) .. controls (262.44,257.09) and (264.65,254.89) .. (267.36,254.89) .. controls (270.08,254.89) and (272.28,257.09) .. (272.28,259.81) .. controls (272.28,262.52) and (270.08,264.72) .. (267.36,264.72) .. controls (264.65,264.72) and (262.44,262.52) .. (262.44,259.81) -- cycle ;
%Straight Lines [id:da15560071721333757] 
\draw    (231.94,239.81) -- (262.44,259.81) ;
%Straight Lines [id:da37378907821910623] 
\draw    (231.94,239.81) -- (262.44,230.14) ;
%Straight Lines [id:da6581406010816668] 
\draw    (231.94,239.81) -- (262.44,199.81) ;
%Straight Lines [id:da3539121107961025] 
\draw    (232.61,199.81) -- (262.44,230.14) ;
%Straight Lines [id:da4924141810504852] 
\draw    (232.61,199.81) -- (262.44,199.81) ;
%Shape: Circle [id:dp34377368464813585] 
\draw   (464.57,181.05) .. controls (464.54,183.77) and (462.31,185.94) .. (459.6,185.91) .. controls (456.88,185.87) and (454.71,183.64) .. (454.74,180.93) .. controls (454.77,178.21) and (457,176.04) .. (459.72,176.07) .. controls (462.43,176.11) and (464.61,178.34) .. (464.57,181.05) -- cycle ;
%Shape: Circle [id:dp9178912133931822] 
\draw   (465.74,141.06) .. controls (465.7,143.78) and (463.47,145.95) .. (460.76,145.92) .. controls (458.04,145.88) and (455.87,143.65) .. (455.9,140.94) .. controls (455.94,138.22) and (458.16,136.05) .. (460.88,136.08) .. controls (463.59,136.12) and (465.77,138.35) .. (465.74,141.06) -- cycle ;
%Shape: Circle [id:dp8351928476259753] 
\draw   (424.54,210.22) .. controls (424.51,212.94) and (422.28,215.11) .. (419.56,215.08) .. controls (416.85,215.04) and (414.68,212.82) .. (414.71,210.1) .. controls (414.74,207.39) and (416.97,205.21) .. (419.69,205.25) .. controls (422.4,205.28) and (424.58,207.51) .. (424.54,210.22) -- cycle ;
%Shape: Circle [id:dp3707905271328862] 
\draw   (424.91,180.56) .. controls (424.88,183.27) and (422.65,185.45) .. (419.93,185.41) .. controls (417.22,185.38) and (415.04,183.15) .. (415.08,180.44) .. controls (415.11,177.72) and (417.34,175.55) .. (420.05,175.58) .. controls (422.77,175.62) and (424.94,177.84) .. (424.91,180.56) -- cycle ;
%Shape: Circle [id:dp5018707566665455] 
\draw   (425.29,150.23) .. controls (425.25,152.94) and (423.02,155.12) .. (420.31,155.08) .. controls (417.59,155.05) and (415.42,152.82) .. (415.45,150.11) .. controls (415.49,147.39) and (417.71,145.22) .. (420.43,145.25) .. controls (423.14,145.28) and (425.32,147.51) .. (425.29,150.23) -- cycle ;
%Shape: Circle [id:dp8856851142674582] 
\draw   (425.65,120.56) .. controls (425.62,123.28) and (423.39,125.45) .. (420.68,125.42) .. controls (417.96,125.39) and (415.79,123.16) .. (415.82,120.44) .. controls (415.85,117.73) and (418.08,115.55) .. (420.8,115.59) .. controls (423.51,115.62) and (425.69,117.85) .. (425.65,120.56) -- cycle ;
%Straight Lines [id:da33529987515225446] 
\draw    (455.9,140.94) -- (425.65,120.56) ;
%Shape: Circle [id:dp5264480345347509] 
\draw   (426.02,91.23) .. controls (425.98,93.95) and (423.75,96.12) .. (421.04,96.09) .. controls (418.32,96.05) and (416.15,93.83) .. (416.18,91.11) .. controls (416.22,88.4) and (418.45,86.22) .. (421.16,86.26) .. controls (423.88,86.29) and (426.05,88.52) .. (426.02,91.23) -- cycle ;
%Straight Lines [id:da157477376639664] 
\draw    (455.9,140.94) -- (425.29,150.23) ;
%Straight Lines [id:da33904003741582134] 
\draw    (455.9,140.94) -- (424.91,180.56) ;
%Straight Lines [id:da5806907313874954] 
\draw    (455.9,140.94) -- (438.1,180.27) -- (424.54,210.22) ;
%Straight Lines [id:da8739031692294434] 
\draw    (454.74,180.93) -- (425.65,120.56) ;
%Straight Lines [id:da27461088325975624] 
\draw    (454.74,180.93) -- (425.29,150.23) ;
%Straight Lines [id:da39564776268820756] 
\draw    (454.74,180.93) -- (424.91,180.56) ;
%Straight Lines [id:da07764437091347598] 
\draw    (454.74,180.93) -- (424.54,210.22) ;
%Straight Lines [id:da5694800500657564] 
\draw    (455.9,140.94) -- (426.02,91.23) ;
%Shape: Circle [id:dp772477570578505] 
\draw   (325.11,21.16) .. controls (325.11,18.44) and (327.31,16.24) .. (330.03,16.24) .. controls (332.74,16.24) and (334.94,18.44) .. (334.94,21.16) .. controls (334.94,23.87) and (332.74,26.07) .. (330.03,26.07) .. controls (327.31,26.07) and (325.11,23.87) .. (325.11,21.16) -- cycle ;
%Shape: Circle [id:dp6727505868534842] 
\draw   (325.44,50.16) .. controls (325.44,47.44) and (327.65,45.24) .. (330.36,45.24) .. controls (333.08,45.24) and (335.28,47.44) .. (335.28,50.16) .. controls (335.28,52.87) and (333.08,55.07) .. (330.36,55.07) .. controls (327.65,55.07) and (325.44,52.87) .. (325.44,50.16) -- cycle ;
%Shape: Circle [id:dp8381762322950737] 
\draw   (325.11,80.49) .. controls (325.11,77.78) and (327.31,75.57) .. (330.03,75.57) .. controls (332.74,75.57) and (334.94,77.78) .. (334.94,80.49) .. controls (334.94,83.21) and (332.74,85.41) .. (330.03,85.41) .. controls (327.31,85.41) and (325.11,83.21) .. (325.11,80.49) -- cycle ;
%Shape: Circle [id:dp35778326895678747] 
\draw   (326.11,199.47) .. controls (326.11,196.76) and (328.31,194.56) .. (331.03,194.56) .. controls (333.74,194.56) and (335.94,196.76) .. (335.94,199.47) .. controls (335.94,202.19) and (333.74,204.39) .. (331.03,204.39) .. controls (328.31,204.39) and (326.11,202.19) .. (326.11,199.47) -- cycle ;
%Shape: Circle [id:dp878861868642367] 
\draw   (326.44,228.47) .. controls (326.44,225.76) and (328.65,223.56) .. (331.36,223.56) .. controls (334.08,223.56) and (336.28,225.76) .. (336.28,228.47) .. controls (336.28,231.19) and (334.08,233.39) .. (331.36,233.39) .. controls (328.65,233.39) and (326.44,231.19) .. (326.44,228.47) -- cycle ;
%Straight Lines [id:da867966675008154] 
\draw    (270.28,24.16) -- (325.11,21.16) ;
%Straight Lines [id:da7502310164293893] 
\draw    (270.28,53.99) -- (325.11,21.16) ;
%Straight Lines [id:da9984745687352241] 
\draw    (270.28,84.16) -- (325.11,21.16) ;
%Straight Lines [id:da4622936699376554] 
\draw    (270.28,53.82) -- (325.44,50.16) ;
%Straight Lines [id:da34892078430157203] 
\draw [line width=0.75]    (270.28,84.16) -- (325.44,50.16) ;
%Straight Lines [id:da8958479647590891] 
\draw    (270.28,84.16) -- (325.44,80.49) ;
%Straight Lines [id:da8832602711727398] 
\draw    (272.28,199.81) -- (326.11,199.47) ;
%Straight Lines [id:da8044072689678781] 
\draw    (272.28,230.14) -- (326.11,199.47) ;
%Straight Lines [id:da19436302835769337] 
\draw    (272.28,230.14) -- (326.44,228.47) ;
%Straight Lines [id:da27767908818889686] 
\draw    (335.28,50.16) -- (416.18,91.11) ;
%Straight Lines [id:da24243738323404584] 
\draw    (334.94,80.49) -- (416.18,91.11) ;
%Straight Lines [id:da13074613110693445] 
\draw    (415.74,91.06) -- (336.28,228.47) ;
%Straight Lines [id:da9433266772103164] 
\draw    (335.28,50.16) -- (415.82,120.44) ;
%Straight Lines [id:da2461825035067009] 
\draw    (334.94,80.49) -- (415.82,120.44) ;
%Straight Lines [id:da48742752264249134] 
\draw    (334.94,80.49) -- (415.45,150.11) ;
%Straight Lines [id:da42228982667891635] 
\draw    (415.45,150.11) -- (336.28,228.47) ;

% Text Node
\draw (257.87,120.51) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{i}^{1}$};
% Text Node
\draw (203.87,83.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{i}^{2}$};
% Text Node
\draw (205.07,46) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{i}^{3}$};
% Text Node
\draw (261.87,267.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{j}^{1}$};
% Text Node
\draw (206.27,233.13) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{j}^{2}$};
% Text Node
\draw (207.87,193.53) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{j}^{3}$};
% Text Node
\draw (261.87,181.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle v_{1}$};
% Text Node
\draw (261.07,211.2) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle v_{2}$};
% Text Node
\draw (259.87,65.2) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle u_{3}$};
% Text Node
\draw (259.07,35.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle u_{2}$};
% Text Node
\draw (259.07,6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle u_{1}$};
% Text Node
\draw (415.07,71.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle e_{1}$};
% Text Node
\draw (415.47,102.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle e_{2}$};
% Text Node
\draw (414.67,131.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle e_{3}$};
% Text Node
\draw (414.27,161.2) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle e_{4}$};
% Text Node
\draw (413.87,216.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{ij}^{1}$};
% Text Node
\draw (466.67,172.67) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{ij}^{2}$};
% Text Node
\draw (468.67,132.27) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle x_{ij}^{3}$};
% Text Node
\draw (337.07,12.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle f_{ij}[ u_{1}]$};
% Text Node
\draw (316.27,87.2) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle f_{ij}[ u_{3}]$};
% Text Node
\draw (320.27,178.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle f_{ij}[ v_{1}]$};
% Text Node
\draw (316.67,234.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle f_{ij}[ v_{2}]$};


\end{tikzpicture}

    


\captionof{figure}{An illustration of the vertex selection gadgets (left) for $V_i = \{u_1, u_2, u_3\}$ and $V_j = \{v_1, v_2\}$
with respect to the fixed ordering, the edge selection gadget (right) for $E_{i.j} = \{e_1, e_2, e_3, e_4\}$ with
$e_1 = u_1v_1, e_2 = u_1v_2, e_3 = u_2v_1, e_4 = u_3v_2$, and their validation gadget (middle)}
\end{frame}
\end{center}
\end{proof}


==> w_hard_general_graph.tex <==
\section{W hard Results}

\begin{lemma}
Perfect Total Domination is W[1] member in General Graph
\end{lemma}
We just follow the proof of Cesati for perfect code \cite{Cesati} and user similar technique as \cite{perf} change only in phase 2 and 3.\\

\begin{proof}


Given a graph $G = (V,E)$, the reduction constructs a non deterministic Turing machine M on empty input such that G has a "perfect code(for our case \ptds)" of k vertices if and only if M has an accepting branch of computation in $k' = f(k)$ steps, for some computable function f. The machine M operates in three phrases.\\

Phase 1. Guess k vertices as the dominating set D.

No change in this step.\\

Phase 2. Check that the k guessed vertices are “perfect” by verifying three conditions:
\begin{enumerate}
    \item For every pair of guessed vertices x and y, x and y are different.
    
    \item  For every pair of guessed vertices x and y, x and y are not adjacent.
    
    \item For every pair of guessed vertices x and y, there is no vertex z $\in$ V that are
adjacent to both x and y.
\end{enumerate}


We just omit condition 2 for \ptds.\\

Phase 3 : Take the sum of the closed neighborhood sizes of the k guessed vertices to verify that the number of dominated vertices is exactly n.

We change that the sum of the open neighborhood sizes of the k guessed vertices should be n for perfect total domination.

Phase 2 grant that no vertex in G belongs to the open neighborhood of two different guessed vertices. In other words, the guessed vertices cover non-overlapping subsets of V: Therefore, the sum cannot be greater than n; moreover, if the sum is equal to n; all vertices in G are dominated by the guessed k-element subset of V.

It is straightforward to verify that the Turing machine T includes $O(n^2)$ instructions, that it can be derived in polynomial time in the size of G; and that it accepts in $O(k^2)$ steps if and only if there exists \ptds of size k in G.

\end{proof}
